Happy Birthday? Age Labels, Search Criteria, and Matching from Dating to Marriage

Age is a match trait and a prominent label on search platforms. Using confidential records from a large Japanese marriage platform, I study how a birthday age update affects consideration, applications, relationship progression, and engagement. Only displayed age updates at birthdays. Receivers enter some acceptable-age ranges as they exit others, leaving only modest overall eligibility changes. Application counts often increase. Applications shift from younger to older suitors. Proposal counts fall at nine of ten female receiver ages \(31\text{--}40\), with losses concentrated at entry into early dating. In stage-specific accounting for receivers in their thirties, the no-birthday proposal count is \(12.9\) percent above the benchmark for female receivers and \(6.7\) percent below it for male receivers; the younger-man share in the female-receiver channel is \(4.8\) percentage points higher. Age labels and filters are not neutral windows onto preferences: they govern who marries whom and how many marriages form.

==> figuretable/birthday_project/assortativeness_likelihood_decomposition.tex <==
\begin{tabular}[t]{lrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Assortativeness Index Levels} & \multicolumn{3}{c}{Decomposition: $I_L(M^+) - I_L(M^-)$} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7}
Receiver Gender & $I_L(M^-)$ & $I_L(M')$ & $I_L(M^+)$ & Total Change & Mechanical & Behavioral\\
\midrule
Female & 2.2534 & 2.2092 [-2.0\%] & 2.2212 [-1.4\%] & -0.0322 & -0.0442 & 0.0120\\
Male & 2.5217 & 1.6192 [-35.8\%] & 1.3093 [-48.1\%] & -1.2124 & -0.9024 & -0.3100\\
\bottomrule
\end{tabular}


==> figuretable/birthday_project/assortativeness_trace_decomposition.tex <==
\begin{tabular}[t]{lrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Assortativeness Index Levels} & \multicolumn{3}{c}{Decomposition: $I(M^+) - I(M^-)$} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7}
Receiver Gender & $I(M^-)$ & $I(M')$ & $I(M^+)$ & Total Change & Mechanical & Behavioral\\
\midrule
Female & 0.0925 & 0.0941 [1.8\%] & 0.0986 [6.6\%] & 0.0061 & 0.0017 & 0.0044\\
Male & 0.1109 & 0.0676 [-39.1\%] & 0.0562 [-49.3\%] & -0.0547 & -0.0433 & -0.0114\\
\bottomrule
\end{tabular}


==> figuretable/birthday_project/eventstudy_proposer_application_results.tex <==

\begin{tabular}[t]{lrrlrrlrrlrrlrrlrrlrrl}
\toprule
Proposer DB & 25 & 26 & 27 & 28 & 29 & 30 & 31 & 32 & 33 & 34 & 35 & 36 & 37 & 38 & 39 & 40 & 41 & 42 & 43 & 44 & 45\\
\midrule
M / Total & 1.61 & 0.61 & -0.38 & 0.16 & 0.00 & -0.09 & 0.02 & 0.03 & 0.11 & 0.07 & -0.08 & -0.05 & 0.21 & 0.06 & -0.16 & -0.39 & -0.03 & 0.11 & 0.05 & 0.01 & -0.11\\
M / Total (SE) & (0.65) & (0.45) & (0.36) & (0.21) & (0.20) & (0.16) & (0.13) & (0.13) & (0.12) & (0.12) & (0.11) & (0.11) & (0.12) & (0.12) & (0.12) & (0.13) & (0.17) & (0.16) & (0.15) & (0.16) & (0.16)\\
M / H Age & 1.07 & 0.47 & -0.18 & 0.13 & 0.04 & 0.04 & 0.12 & 0.06 & 0.04 & 0.02 & -0.01 & 0.01 & -0.01 & 0.04 & 0.01 & -0.00 & 0.00 & 0.00 & 0.01 & 0.02 & 0.02\\
M / H Age (SE) & (0.52) & (0.29) & (0.25) & (0.11) & (0.10) & (0.07) & (0.06) & (0.04) & (0.03) & (0.03) & (0.02) & (0.02) & (0.02) & (0.02) & (0.01) & (0.02) & (0.01) & (0.01) & (0.01) & (0.01) & (0.02)\\
M / L Age & 0.22 & 0.09 & -0.12 & -0.05 & -0.08 & -0.17 & -0.10 & -0.04 & 0.07 & 0.02 & -0.08 & -0.07 & 0.19 & 0.01 & -0.18 & -0.39 & -0.04 & 0.08 & 0.02 & -0.02 & -0.15\\
M / L Age (SE) & (0.12) & (0.14) & (0.10) & (0.09) & (0.10) & (0.09) & (0.08) & (0.09) & (0.09) & (0.10) & (0.09) & (0.09) & (0.11) & (0.11) & (0.11) & (0.12) & (0.16) & (0.15) & (0.14) & (0.15) & (0.15)\\
M / H Income & 0.33 & 0.06 & -0.10 & 0.06 & -0.01 & 0.00 & 0.02 & -0.00 & 0.01 & 0.04 & -0.01 & 0.02 & 0.07 & 0.03 & -0.02 & -0.06 & -0.00 & 0.05 & 0.03 & 0.06 & -0.02\\
M / H Income (SE) & (0.11) & (0.09) & (0.07) & (0.03) & (0.03) & (0.03) & (0.03) & (0.03) & (0.02) & (0.03) & (0.02) & (0.02) & (0.03) & (0.03) & (0.03) & (0.03) & (0.04) & (0.04) & (0.04) & (0.05) & (0.05)\\
M / L Income & 1.27 & 0.55 & -0.27 & 0.11 & 0.01 & -0.09 & -0.00 & 0.03 & 0.10 & 0.03 & -0.07 & -0.07 & 0.14 & 0.04 & -0.14 & -0.33 & -0.03 & 0.05 & 0.01 & -0.05 & -0.10\\
M / L Income (SE) & (0.57) & (0.41) & (0.30) & (0.19) & (0.18) & (0.15) & (0.12) & (0.11) & (0.10) & (0.10) & (0.09) & (0.09) & (0.10) & (0.10) & (0.10) & (0.10) & (0.14) & (0.13) & (0.12) & (0.12) & (0.13)\\
M / H Height & 1.05 & 0.38 & -0.31 & 0.13 & -0.02 & -0.06 & 0.01 & 0.01 & 0.10 & 0.07 & -0.04 & -0.02 & 0.16 & 0.06 & -0.14 & -0.31 & -0.02 & 0.08 & 0.02 & 0.04 & -0.12\\
M / H Height (SE) & (0.51) & (0.33) & (0.27) & (0.16) & (0.16) & (0.13) & (0.10) & (0.10) & (0.09) & (0.10) & (0.08) & (0.08) & (0.09) & (0.09) & (0.10) & (0.10) & (0.13) & (0.13) & (0.12) & (0.13) & (0.13)\\
M / L Height & 0.56 & 0.23 & -0.07 & 0.03 & 0.02 & -0.03 & 0.01 & 0.02 & 0.01 & -0.00 & -0.04 & -0.02 & 0.06 & 0.01 & -0.02 & -0.07 & -0.01 & 0.02 & 0.03 & -0.02 & -0.00\\
M / L Height (SE) & (0.18) & (0.14) & (0.10) & (0.06) & (0.05) & (0.05) & (0.03) & (0.03) & (0.03) & (0.03) & (0.03) & (0.03) & (0.03) & (0.03) & (0.03) & (0.03) & (0.04) & (0.04) & (0.04) & (0.04) & (0.04)\\
F / Total & 0.34 & 0.23 & 0.10 & 0.14 & -0.02 & -0.09 & -0.04 & 0.04 & -0.05 & -0.11 & -0.31 & -0.27 & -0.16 & -0.33 & -0.30 & -0.53 & -0.31 & -0.33 & -0.08 & -0.12 & -0.07\\
F / Total (SE) & (0.18) & (0.13) & (0.10) & (0.10) & (0.08) & (0.07) & (0.08) & (0.07) & (0.07) & (0.07) & (0.07) & (0.07) & (0.08) & (0.08) & (0.09) & (0.10) & (0.10) & (0.11) & (0.12) & (0.13) & (0.13)\\
F / H Age & 0.33 & 0.22 & 0.09 & 0.12 & -0.01 & -0.02 & 0.01 & 0.05 & -0.01 & 0.02 & -0.14 & -0.06 & -0.02 & -0.09 & -0.10 & -0.13 & -0.07 & -0.07 & 0.01 & 0.06 & 0.01\\
F / H Age (SE) & (0.18) & (0.12) & (0.09) & (0.08) & (0.06) & (0.05) & (0.06) & (0.05) & (0.05) & (0.05) & (0.04) & (0.04) & (0.05) & (0.05) & (0.05) & (0.06) & (0.06) & (0.06) & (0.07) & (0.07) & (0.07)\\
F / L Age & 0.00 & 0.00 & 0.00 & -0.01 & -0.02 & -0.05 & -0.05 & -0.01 & -0.04 & -0.11 & -0.15 & -0.17 & -0.14 & -0.21 & -0.18 & -0.36 & -0.21 & -0.24 & -0.09 & -0.20 & -0.11\\
F / L Age (SE) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.02) & (0.02) & (0.03) & (0.03) & (0.03) & (0.03) & (0.03) & (0.03) & (0.04) & (0.04) & (0.05) & (0.06) & (0.06) & (0.07) & (0.06)\\
F / H Income & 0.23 & 0.13 & 0.10 & 0.10 & -0.02 & -0.07 & -0.02 & 0.02 & -0.03 & -0.08 & -0.26 & -0.22 & -0.15 & -0.28 & -0.26 & -0.44 & -0.29 & -0.28 & -0.06 & -0.12 & -0.10\\
F / H Income (SE) & (0.14) & (0.09) & (0.07) & (0.07) & (0.06) & (0.05) & (0.06) & (0.06) & (0.06) & (0.06) & (0.06) & (0.06) & (0.06) & (0.07) & (0.08) & (0.09) & (0.09) & (0.10) & (0.11) & (0.12) & (0.11)\\
F / L Income & 0.11 & 0.10 & 0.00 & 0.03 & -0.00 & -0.02 & -0.02 & 0.02 & -0.02 & -0.03 & -0.05 & -0.05 & -0.00 & -0.04 & -0.04 & -0.08 & -0.02 & -0.05 & -0.01 & -0.01 & 0.00\\
F / L Income (SE) & (0.07) & (0.06) & (0.04) & (0.04) & (0.03) & (0.02) & (0.03) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.03) & (0.03)\\
F / H Height & 0.27 & 0.18 & 0.09 & 0.12 & -0.01 & -0.10 & -0.04 & 0.06 & -0.04 & -0.09 & -0.27 & -0.23 & -0.14 & -0.26 & -0.24 & -0.39 & -0.24 & -0.26 & -0.05 & -0.11 & -0.07\\
F / H Height (SE) & (0.14) & (0.10) & (0.08) & (0.08) & (0.06) & (0.06) & (0.06) & (0.06) & (0.06) & (0.06) & (0.06) & (0.06) & (0.06) & (0.07) & (0.07) & (0.08) & (0.08) & (0.09) & (0.10) & (0.10) & (0.10)\\
F / L Height & 0.07 & 0.05 & 0.01 & 0.02 & -0.01 & 0.01 & -0.00 & -0.02 & -0.01 & -0.02 & -0.04 & -0.05 & -0.02 & -0.06 & -0.06 & -0.13 & -0.07 & -0.07 & -0.02 & -0.02 & -0.02\\
F / L Height (SE) & (0.05) & (0.03) & (0.03) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.03) & (0.03) & (0.03) & (0.04) & (0.03)\\
\bottomrule
\end{tabular}


==> figuretable/birthday_project/eventstudy_proposer_prerelation_results.tex <==

\begin{tabular}[t]{lrrlrrlrrlrrlrrlrrlrrl}
\toprule
Proposer DB & 25 & 26 & 27 & 28 & 29 & 30 & 31 & 32 & 33 & 34 & 35 & 36 & 37 & 38 & 39 & 40 & 41 & 42 & 43 & 44 & 45\\
\midrule
M / Total & 0.02 & -0.01 & -0.01 & 0.01 & -0.02 & -0.01 & 0.00 & -0.00 & -0.01 & -0.01 & -0.00 & 0.00 & -0.00 & -0.00 & -0.01 & -0.01 & -0.00 & 0.00 & -0.00 & -0.00 & -0.01\\
M / Total (SE) & (0.03) & (0.02) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.01) & (0.00)\\
M / H Age & 0.01 & -0.01 & -0.00 & 0.01 & -0.00 & -0.00 & 0.01 & 0.00 & 0.00 & -0.00 & -0.00 & 0.00 & -0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -0.00 & 0.00 & 0.00 & -0.00\\
M / H Age (SE) & (0.03) & (0.02) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
M / L Age & 0.01 & -0.00 & 0.00 & 0.00 & -0.01 & -0.01 & -0.00 & -0.00 & -0.01 & -0.01 & -0.01 & -0.00 & -0.01 & -0.00 & -0.01 & -0.01 & -0.00 & 0.00 & -0.00 & -0.00 & -0.01\\
M / L Age (SE) & (0.02) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.01) & (0.00)\\
M / H Income & -0.01 & -0.00 & -0.00 & -0.00 & -0.01 & -0.00 & 0.00 & 0.00 & -0.00 & -0.00 & 0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & 0.00 & 0.00 & -0.00 & -0.00\\
M / H Income (SE) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
M / L Income & 0.03 & -0.00 & -0.01 & 0.01 & -0.01 & -0.00 & 0.00 & -0.01 & -0.00 & -0.01 & -0.01 & 0.00 & -0.00 & 0.00 & -0.01 & -0.01 & -0.00 & 0.00 & -0.01 & -0.00 & -0.00\\
M / L Income (SE) & (0.03) & (0.02) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
M / H Height & 0.01 & -0.01 & -0.00 & 0.00 & -0.01 & -0.01 & -0.00 & -0.00 & -0.01 & -0.01 & -0.00 & 0.00 & -0.00 & -0.00 & -0.01 & -0.01 & -0.00 & 0.00 & 0.00 & -0.00 & -0.01\\
M / H Height (SE) & (0.03) & (0.02) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
M / L Height & 0.01 & 0.00 & -0.00 & 0.01 & -0.00 & 0.00 & 0.01 & 0.00 & -0.00 & -0.00 & -0.00 & 0.00 & -0.00 & 0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & 0.00\\
M / L Height (SE) & (0.01) & (0.01) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
F / Total & 0.01 & 0.02 & -0.00 & -0.00 & -0.01 & -0.00 & -0.00 & -0.00 & -0.01 & -0.00 & -0.01 & -0.01 & -0.01 & -0.01 & -0.01 & -0.02 & -0.00 & -0.01 & -0.00 & -0.00 & -0.00\\
F / Total (SE) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.01) & (0.01) & (0.01) & (0.01)\\
F / H Age & 0.01 & 0.02 & 0.00 & 0.00 & -0.00 & -0.00 & -0.00 & 0.00 & -0.00 & 0.00 & -0.01 & -0.01 & -0.00 & -0.00 & -0.00 & -0.01 & -0.00 & -0.01 & 0.00 & 0.00 & 0.00\\
F / H Age (SE) & (0.01) & (0.01) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.01)\\
F / L Age & -0.00 & 0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.01 & -0.01 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.01 & -0.01 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00\\
F / L Age (SE) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
F / H Income & 0.01 & 0.01 & -0.01 & 0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.01 & -0.00 & -0.01 & -0.01 & -0.00 & -0.01 & -0.01 & -0.01 & -0.00 & -0.01 & -0.00 & -0.00 & -0.00\\
F / H Income (SE) & (0.01) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
F / L Income & -0.00 & 0.01 & 0.00 & -0.00 & -0.01 & -0.00 & -0.00 & -0.00 & 0.00 & -0.00 & -0.01 & -0.00 & -0.00 & -0.00 & -0.00 & -0.01 & 0.00 & -0.00 & -0.00 & 0.00 & 0.00\\
F / L Income (SE) & (0.01) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
F / H Height & 0.01 & 0.02 & 0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.01 & 0.00 & -0.01 & -0.01 & -0.01 & -0.00 & -0.01 & -0.01 & -0.00 & -0.01 & 0.00 & -0.00 & -0.00\\
F / H Height (SE) & (0.01) & (0.01) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
F / L Height & -0.00 & 0.00 & -0.00 & -0.00 & -0.01 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.01 & 0.00 & -0.00 & -0.00 & -0.00 & 0.00\\
F / L Height (SE) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
\bottomrule
\end{tabular}


==> figuretable/birthday_project/eventstudy_receiver_application_results.tex <==

\begin{tabular}[t]{lrrlrrlrrlrrlrrlrrlrrl}
\toprule
Receiver DB & 25 & 26 & 27 & 28 & 29 & 30 & 31 & 32 & 33 & 34 & 35 & 36 & 37 & 38 & 39 & 40 & 41 & 42 & 43 & 44 & 45\\
\midrule
M / Total & 0.20 & 0.24 & 0.29 & 0.34 & 0.14 & 0.32 & 0.12 & 0.23 & 0.12 & 0.21 & 0.19 & 0.04 & 0.07 & 0.28 & -0.00 & 0.03 & -0.07 & 0.04 & -0.06 & -0.10 & -0.12\\
M / Total (SE) & (0.11) & (0.07) & (0.06) & (0.08) & (0.07) & (0.07) & (0.07) & (0.08) & (0.08) & (0.08) & (0.06) & (0.07) & (0.06) & (0.07) & (0.06) & (0.06) & (0.06) & (0.05) & (0.04) & (0.04) & (0.04)\\
M / H Age & 0.10 & 0.21 & 0.20 & 0.29 & 0.14 & 0.34 & 0.14 & 0.21 & 0.19 & 0.23 & 0.27 & 0.19 & 0.20 & 0.22 & 0.13 & 0.17 & 0.06 & 0.06 & 0.06 & 0.04 & 0.06\\
M / H Age (SE) & (0.07) & (0.05) & (0.04) & (0.05) & (0.04) & (0.03) & (0.03) & (0.03) & (0.02) & (0.02) & (0.02) & (0.02) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01)\\
M / M Age & 0.09 & 0.03 & 0.07 & 0.03 & 0.08 & 0.06 & 0.05 & 0.08 & 0.07 & 0.11 & 0.09 & 0.09 & 0.10 & 0.10 & 0.09 & 0.08 & 0.04 & 0.06 & 0.04 & 0.03 & 0.02\\
M / M Age (SE) & (0.04) & (0.02) & (0.02) & (0.02) & (0.02) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01)\\
M / L Age & 0.01 & -0.00 & 0.02 & 0.01 & -0.08 & -0.08 & -0.06 & -0.06 & -0.14 & -0.13 & -0.16 & -0.23 & -0.22 & -0.04 & -0.22 & -0.22 & -0.17 & -0.08 & -0.16 & -0.18 & -0.20\\
M / L Age (SE) & (0.03) & (0.03) & (0.02) & (0.03) & (0.04) & (0.04) & (0.04) & (0.04) & (0.05) & (0.05) & (0.05) & (0.05) & (0.04) & (0.05) & (0.05) & (0.05) & (0.05) & (0.04) & (0.04) & (0.04) & (0.04)\\
M / H Income & 0.00 & 0.03 & 0.02 & 0.04 & 0.04 & 0.07 & 0.02 & 0.07 & 0.04 & 0.04 & 0.07 & 0.06 & 0.04 & 0.07 & 0.01 & -0.00 & -0.01 & 0.02 & -0.00 & -0.04 & -0.05\\
M / H Income (SE) & (0.02) & (0.01) & (0.01) & (0.01) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02)\\
M / L Income & 0.19 & 0.21 & 0.27 & 0.30 & 0.10 & 0.24 & 0.10 & 0.16 & 0.08 & 0.16 & 0.12 & -0.02 & 0.03 & 0.21 & -0.01 & 0.04 & -0.06 & 0.01 & -0.06 & -0.06 & -0.07\\
M / L Income (SE) & (0.10) & (0.07) & (0.05) & (0.08) & (0.06) & (0.06) & (0.06) & (0.07) & (0.07) & (0.06) & (0.05) & (0.05) & (0.04) & (0.05) & (0.04) & (0.04) & (0.04) & (0.03) & (0.03) & (0.03) & (0.03)\\
M / H Height & 0.13 & 0.19 & 0.19 & 0.27 & 0.15 & 0.25 & 0.10 & 0.19 & 0.09 & 0.16 & 0.15 & 0.03 & 0.06 & 0.22 & 0.01 & 0.03 & -0.05 & 0.03 & -0.04 & -0.07 & -0.09\\
M / H Height (SE) & (0.09) & (0.06) & (0.05) & (0.07) & (0.06) & (0.06) & (0.06) & (0.06) & (0.06) & (0.06) & (0.05) & (0.05) & (0.04) & (0.05) & (0.05) & (0.05) & (0.05) & (0.04) & (0.04) & (0.03) & (0.03)\\
M / L Height & 0.06 & 0.05 & 0.10 & 0.07 & -0.01 & 0.07 & 0.02 & 0.04 & 0.03 & 0.05 & 0.04 & 0.01 & 0.01 & 0.06 & -0.01 & 0.01 & -0.02 & 0.01 & -0.02 & -0.02 & -0.03\\
M / L Height (SE) & (0.04) & (0.03) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.01) & (0.02) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01)\\
F / Total & 0.81 & 0.31 & 0.39 & 0.47 & 0.27 & 0.26 & 0.04 & 0.22 & 0.17 & 0.22 & 0.39 & 0.19 & 0.38 & 0.34 & -0.02 & 0.34 & -0.01 & -0.05 & -0.02 & 0.07 & 0.16\\
F / Total (SE) & (0.23) & (0.18) & (0.14) & (0.12) & (0.09) & (0.09) & (0.08) & (0.09) & (0.08) & (0.07) & (0.07) & (0.06) & (0.06) & (0.06) & (0.07) & (0.06) & (0.06) & (0.07) & (0.06) & (0.05) & (0.06)\\
F / H Age & 0.80 & 0.39 & 0.46 & 0.55 & 0.37 & 0.43 & 0.18 & 0.32 & 0.33 & 0.39 & 0.54 & 0.33 & 0.49 & 0.45 & 0.11 & 0.47 & 0.06 & 0.02 & 0.05 & 0.13 & 0.21\\
F / H Age (SE) & (0.23) & (0.17) & (0.13) & (0.11) & (0.08) & (0.08) & (0.07) & (0.07) & (0.07) & (0.06) & (0.06) & (0.06) & (0.06) & (0.06) & (0.06) & (0.06) & (0.05) & (0.06) & (0.05) & (0.05) & (0.05)\\
F / M Age & 0.03 & -0.02 & -0.01 & -0.01 & -0.01 & -0.01 & -0.01 & -0.00 & -0.02 & -0.02 & -0.02 & -0.01 & -0.01 & -0.02 & -0.02 & -0.02 & -0.01 & -0.01 & -0.01 & -0.01 & -0.00\\
F / M Age (SE) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.00) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01)\\
F / L Age & -0.02 & -0.06 & -0.05 & -0.07 & -0.10 & -0.15 & -0.13 & -0.10 & -0.14 & -0.15 & -0.13 & -0.13 & -0.10 & -0.09 & -0.10 & -0.11 & -0.06 & -0.07 & -0.06 & -0.05 & -0.05\\
F / L Age (SE) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01)\\
F / H Income & 0.28 & 0.18 & 0.19 & 0.25 & 0.20 & 0.15 & 0.06 & 0.18 & 0.13 & 0.14 & 0.20 & 0.10 & 0.21 & 0.21 & -0.02 & 0.14 & 0.02 & -0.07 & -0.01 & 0.02 & 0.01\\
F / H Income (SE) & (0.16) & (0.11) & (0.09) & (0.07) & (0.06) & (0.06) & (0.05) & (0.06) & (0.05) & (0.05) & (0.05) & (0.04) & (0.04) & (0.04) & (0.04) & (0.04) & (0.04) & (0.05) & (0.04) & (0.03) & (0.04)\\
F / L Income & 0.52 & 0.13 & 0.20 & 0.22 & 0.07 & 0.11 & -0.02 & 0.04 & 0.04 & 0.09 & 0.19 & 0.10 & 0.17 & 0.13 & -0.00 & 0.20 & -0.02 & 0.01 & -0.00 & 0.05 & 0.15\\
F / L Income (SE) & (0.10) & (0.08) & (0.07) & (0.05) & (0.04) & (0.04) & (0.03) & (0.03) & (0.03) & (0.03) & (0.03) & (0.02) & (0.03) & (0.03) & (0.03) & (0.03) & (0.03) & (0.03) & (0.03) & (0.03) & (0.03)\\
F / H Height & 0.50 & 0.24 & 0.25 & 0.31 & 0.17 & 0.16 & 0.04 & 0.16 & 0.09 & 0.15 & 0.24 & 0.12 & 0.22 & 0.18 & -0.05 & 0.18 & 0.01 & -0.05 & -0.06 & 0.06 & 0.06\\
F / H Height (SE) & (0.17) & (0.12) & (0.10) & (0.08) & (0.07) & (0.06) & (0.06) & (0.06) & (0.05) & (0.05) & (0.05) & (0.04) & (0.04) & (0.04) & (0.05) & (0.04) & (0.04) & (0.05) & (0.04) & (0.03) & (0.04)\\
F / L Height & 0.30 & 0.08 & 0.14 & 0.16 & 0.10 & 0.11 & 0.00 & 0.06 & 0.08 & 0.07 & 0.15 & 0.07 & 0.16 & 0.16 & 0.03 & 0.16 & -0.02 & -0.01 & 0.04 & 0.02 & 0.10\\
F / L Height (SE) & (0.08) & (0.06) & (0.05) & (0.04) & (0.03) & (0.03) & (0.03) & (0.03) & (0.03) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) & (0.03) & (0.03) & (0.02) & (0.03) & (0.03) & (0.02) & (0.03)\\
\bottomrule
\end{tabular}


==> figuretable/birthday_project/eventstudy_receiver_prerelation_results.tex <==

\begin{tabular}[t]{lrrlrrlrrlrrlrrlrrlrrl}
\toprule
Receiver DB & 25 & 26 & 27 & 28 & 29 & 30 & 31 & 32 & 33 & 34 & 35 & 36 & 37 & 38 & 39 & 40 & 41 & 42 & 43 & 44 & 45\\
\midrule
M / Total & 0.03 & -0.01 & 0.02 & 0.02 & 0.01 & 0.00 & 0.01 & 0.01 & 0.00 & 0.00 & 0.01 & -0.00 & 0.01 & -0.00 & -0.01 & -0.00 & -0.01 & 0.00 & 0.00 & 0.00 & -0.00\\
M / Total (SE) & (0.02) & (0.02) & (0.01) & (0.01) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
M / H Age & 0.02 & -0.01 & 0.01 & 0.01 & 0.00 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\
M / H Age (SE) & (0.02) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
M / M Age & 0.00 & -0.00 & 0.01 & 0.00 & 0.01 & -0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -0.00 & -0.00 & 0.00 & 0.00 & 0.00 & 0.00\\
M / M Age (SE) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
M / L Age & 0.01 & 0.00 & 0.00 & 0.01 & 0.00 & -0.00 & 0.00 & 0.00 & -0.00 & 0.00 & -0.00 & -0.01 & 0.00 & -0.00 & -0.01 & -0.00 & -0.01 & 0.00 & -0.00 & -0.00 & -0.00\\
M / L Age (SE) & (0.01) & (0.01) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
M / H Income & NA & -0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -0.00 & 0.00 & -0.00 & 0.00 & 0.00 & 0.00 & -0.00 & 0.00 & 0.00 & 0.00 & -0.00 & -0.00 & -0.00\\
M / H Income (SE) & (NA) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
M / L Income & 0.03 & -0.01 & 0.02 & 0.02 & 0.01 & -0.00 & 0.01 & 0.01 & 0.00 & 0.00 & 0.01 & -0.00 & 0.00 & -0.00 & -0.00 & -0.00 & -0.01 & 0.00 & 0.00 & 0.00 & -0.00\\
M / L Income (SE) & (0.02) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
M / H Height & 0.02 & -0.00 & 0.02 & 0.02 & 0.01 & -0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -0.00 & -0.00 & -0.01 & -0.01 & 0.00 & 0.00 & 0.00 & -0.00\\
M / H Height (SE) & (0.02) & (0.01) & (0.01) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
M / L Height & 0.01 & -0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & -0.00 & 0.00 & 0.00 & -0.00 & 0.00 & 0.00 & -0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -0.00\\
M / L Height (SE) & (0.01) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
F / Total & 0.00 & 0.02 & 0.01 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & -0.00 & -0.00 & -0.00 & -0.00 & 0.00 & -0.01 & -0.01 & -0.01 & 0.00 & -0.00 & 0.00 & -0.00 & -0.00\\
F / Total (SE) & (0.01) & (0.01) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
F / H Age & 0.00 & 0.02 & 0.01 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -0.00 & -0.00 & -0.00 & 0.00 & -0.00 & 0.00 & -0.00 & -0.00\\
F / H Age (SE) & (0.01) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
F / M Age & 0.00 & 0.00 & 0.00 & -0.00 & -0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -0.00 & -0.00 & -0.00 & 0.00 & -0.00 & -0.00 & -0.00 & 0.00 & -0.00 & 0.00 & -0.00 & -0.00\\
F / M Age (SE) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
F / L Age & -0.00 & -0.00 & -0.00 & 0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & 0.00 & -0.00 & -0.00 & 0.00\\
F / L Age (SE) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
F / H Income & -0.00 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -0.00 & -0.00 & 0.00 & -0.00 & -0.01 & -0.01 & -0.00 & 0.00 & -0.00 & 0.00 & -0.00 & -0.00\\
F / H Income (SE) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
F / L Income & 0.01 & 0.01 & -0.00 & -0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -0.00 & 0.00 & 0.00 & -0.00 & 0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & 0.00 & -0.00 & 0.00\\
F / L Income (SE) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
F / H Height & -0.00 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.01 & -0.00 & -0.01 & 0.00 & -0.00 & 0.00 & -0.00 & -0.00\\
F / H Height (SE) & (0.01) & (0.01) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
F / L Height & 0.00 & 0.01 & 0.00 & -0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -0.00 & 0.00 & 0.00 & 0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & -0.00 & 0.00\\
F / L Height (SE) & (0.01) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00) & (0.00)\\
\bottomrule
\end{tabular}


==> figuretable/birthday_project/ttest_receiver_proposal_results.tex <==

\begin{tabular}[t]{lrrlrrlrrlrrlrrlrrlrrl}
\toprule
Receiver DB (Proposal) & 25 & 26 & 27 & 28 & 29 & 30 & 31 & 32 & 33 & 34 & 35 & 36 & 37 & 38 & 39 & 40 & 41 & 42 & 43 & 44 & 45\\
\midrule
M / Total & 0.33 & 0.22 & 0.56 & 0.33 & 1.78 & -1.89 & -1.11 & 1.89 & 0.56 & 1.89 & 1.44 & -0.44 & -0.44 & 3.33 & 0.67 & -4.00 & -2.67 & 2.56 & 0.78 & 1.78 & -0.44\\
M / Total (p) & (0.166) & (0.587) & (0.381) & (0.728) & (0.144) & (0.243) & (0.500) & (0.275) & (0.747) & (0.249) & (0.409) & (0.793) & (0.758) & (0.016) & (0.688) & (0.009) & (0.015) & (0.039) & (0.536) & (0.305) & (0.766)\\
M / H Age & 0.33 & 0.00 & -0.33 & 0.67 & 0.56 & 0.56 & 1.00 & 0.33 & -0.11 & 1.00 & 0.89 & 0.56 & 1.11 & 0.33 & 0.78 & -0.11 & -0.22 & -0.11 & 0.00 & -0.33 & 0.22\\
M / H Age (p) & (0.132) & (1.000) & (0.468) & (0.325) & (0.210) & (0.396) & (0.102) & (0.602) & (0.862) & (0.065) & (0.048) & (0.272) & (0.055) & (0.332) & (0.015) & (0.347) & (0.411) & (0.624) & (1.000) & (0.132) & (0.169)\\
M / NA & 0.11 & 0.00 & -0.11 & 0.11 & -0.11 & 0.00 & 0.22 & 0.22 & 0.56 & 0.11 & 0.22 & -0.11 & 0.11 & 0.89 & -0.44 & -0.44 & 0.11 & 0.56 & 0.22 & 0.78 & 0.11\\
M / NA (p) & (0.347) & (1.000) & (0.624) & (0.797) & (0.776) & (1.000) & (0.723) & (0.670) & (0.426) & (0.861) & (0.695) & (0.853) & (0.747) & (0.048) & (0.363) & (0.376) & (0.695) & (0.015) & (0.567) & (0.023) & (0.556)\\
M / L Age & -0.11 & 0.22 & 1.00 & -0.44 & 1.33 & -2.44 & -2.33 & 1.33 & 0.11 & 0.78 & 0.33 & -0.89 & -1.67 & 2.11 & 0.33 & -3.44 & -2.56 & 2.11 & 0.56 & 1.33 & -0.78\\
M / L Age (p) & (0.347) & (0.462) & (0.040) & (0.429) & (0.180) & (0.046) & (0.049) & (0.378) & (0.929) & (0.652) & (0.820) & (0.561) & (0.306) & (0.139) & (0.813) & (0.019) & (0.014) & (0.084) & (0.640) & (0.398) & (0.609)\\
M / H Income & 0.00 & 0.00 & 0.11 & 0.22 & 0.44 & -0.11 & 0.11 & -0.33 & 0.00 & -0.11 & 0.33 & -0.44 & -0.11 & 0.78 & 0.44 & -0.56 & -0.33 & 0.89 & 0.22 & 1.11 & 0.11\\
M / H Income (p) &  &  & (0.347) & (0.411) & (0.195) & (0.785) & (0.765) & (0.504) & (1.000) & (0.855) & (0.559) & (0.314) & (0.861) & (0.283) & (0.692) & (0.452) & (0.565) & (0.161) & (0.646) & (0.140) & (0.888)\\
M / L Income & 0.33 & 0.22 & 0.44 & 0.11 & 1.33 & -1.78 & -1.11 & 2.22 & 0.33 & 2.00 & 1.11 & 0.00 & -0.44 & 2.56 & 0.22 & -3.33 & -2.44 & 1.67 & 0.56 & 0.56 & -0.56\\
M / L Income (p) & (0.166) & (0.587) & (0.485) & (0.911) & (0.269) & (0.240) & (0.499) & (0.208) & (0.833) & (0.249) & (0.460) & (1.000) & (0.785) & (0.029) & (0.830) & (0.026) & (0.019) & (0.094) & (0.656) & (0.704) & (0.631)\\
M / H Height & 0.22 & 0.22 & 0.89 & 0.78 & 0.89 & -2.11 & -1.44 & 2.00 & 1.00 & 1.78 & 0.67 & -1.00 & -1.67 & 3.11 & 0.56 & -2.67 & -3.33 & 2.00 & 0.89 & 2.00 & -0.11\\
M / H Height (p) & (0.347) & (0.536) & (0.125) & (0.279) & (0.322) & (0.107) & (0.289) & (0.201) & (0.435) & (0.236) & (0.701) & (0.500) & (0.197) & (0.008) & (0.719) & (0.053) & (0.002) & (0.065) & (0.420) & (0.226) & (0.934)\\
M / L Height & 0.11 & 0.00 & -0.33 & -0.44 & 0.89 & 0.22 & 0.33 & -0.11 & -0.44 & 0.11 & 0.78 & 0.56 & 1.22 & 0.22 & 0.11 & -1.33 & 0.67 & 0.56 & -0.11 & -0.22 & -0.33\\
M / L Height (p) & (0.347) & (1.000) & (0.371) & (0.343) & (0.232) & (0.714) & (0.604) & (0.905) & (0.606) & (0.882) & (0.289) & (0.395) & (0.083) & (0.739) & (0.894) & (0.072) & (0.294) & (0.484) & (0.879) & (0.769) & (0.527)\\
F / Total & 0.89 & 0.89 & 0.89 & 0.56 & 0.89 & 0.89 & -1.44 & -1.11 & 0.33 & 1.22 & -4.00 & -3.44 & -3.22 & -2.11 & -0.67 & -0.44 & -1.22 & -0.22 & 0.00 & -1.89 & 0.22\\
F / Total (p) & (0.253) & (0.315) & (0.464) & (0.731) & (0.679) & (0.541) & (0.297) & (0.588) & (0.892) & (0.400) & (0.045) & (0.005) & (0.071) & (0.114) & (0.689) & (0.715) & (0.409) & (0.797) & (1.000) & (0.083) & (0.676)\\
F / H Age & 0.67 & 0.78 & 0.33 & -0.33 & 0.11 & 1.22 & -1.44 & -0.22 & 2.11 & 1.67 & -1.44 & -3.11 & -2.56 & -1.44 & -0.22 & -0.44 & -0.44 & -0.33 & -0.33 & -1.22 & 0.33\\
F / H Age (p) & (0.409) & (0.351) & (0.811) & (0.832) & (0.955) & (0.354) & (0.278) & (0.890) & (0.189) & (0.253) & (0.438) & (0.032) & (0.069) & (0.249) & (0.895) & (0.728) & (0.670) & (0.696) & (0.715) & (0.161) & (0.530)\\
F / NA & 0.22 & 0.00 & 0.56 & 0.44 & 0.89 & 0.22 & 0.67 & 0.22 & -1.11 & 0.78 & -1.56 & 0.22 & 0.67 & -0.22 & 0.00 & 0.11 & -0.11 & 0.11 & 0.22 & 0.11 & 0.22\\
F / NA (p) & (0.169) & (1.000) & (0.358) & (0.275) & (0.055) & (0.665) & (0.282) & (0.769) & (0.038) & (0.168) & (0.018) & (0.661) & (0.283) & (0.724) & (1.000) & (0.869) & (0.811) & (0.711) & (0.447) & (0.663) & (0.411)\\
F / L Age & 0.00 & 0.11 & 0.00 & 0.44 & -0.11 & -0.56 & -0.67 & -1.11 & -0.67 & -1.22 & -1.00 & -0.56 & -1.33 & -0.44 & -0.44 & -0.11 & -0.67 & 0.00 & 0.11 & -0.78 & -0.33\\
F / L Age (p) &  & (0.556) & (1.000) & (0.314) & (0.846) & (0.401) & (0.448) & (0.098) & (0.437) & (0.099) & (0.126) & (0.572) & (0.083) & (0.399) & (0.256) & (0.862) & (0.095) & (1.000) & (0.862) & (0.140) & (0.260)\\
F / H Income & 0.11 & 0.33 & 1.00 & -1.44 & 0.56 & 1.11 & -1.22 & -2.00 & 1.56 & 1.89 & -1.00 & -3.78 & -1.78 & -0.67 & 0.11 & 0.11 & -0.11 & 0.33 & -0.67 & -0.78 & 0.44\\
F / H Income (p) & (0.855) & (0.646) & (0.233) & (0.061) & (0.596) & (0.391) & (0.246) & (0.127) & (0.347) & (0.135) & (0.434) & (0.006) & (0.248) & (0.499) & (0.911) & (0.890) & (0.913) & (0.646) & (0.390) & (0.322) & (0.277)\\
F / L Income & 0.78 & 0.56 & -0.11 & 1.89 & 0.33 & -0.22 & -0.22 & 0.89 & -1.22 & -0.67 & -3.00 & 0.33 & -1.33 & -1.44 & -0.78 & -0.56 & -1.11 & -0.56 & 0.67 & -1.11 & -0.22\\
F / L Income (p) & (0.070) & (0.513) & (0.903) & (0.144) & (0.805) & (0.866) & (0.800) & (0.527) & (0.362) & (0.637) & (0.021) & (0.701) & (0.102) & (0.188) & (0.469) & (0.506) & (0.146) & (0.507) & (0.516) & (0.148) & (0.551)\\
F / H Height & 0.67 & 1.56 & 1.22 & 0.67 & 1.89 & 0.33 & 0.00 & 0.33 & 1.22 & 0.89 & -3.78 & -2.78 & -2.00 & -0.89 & -0.22 & -0.56 & 0.00 & -0.33 & 0.00 & -1.33 & 0.22\\
F / H Height (p) & (0.348) & (0.068) & (0.203) & (0.607) & (0.312) & (0.824) & (1.000) & (0.836) & (0.509) & (0.514) & (0.010) & (0.024) & (0.173) & (0.454) & (0.837) & (0.415) & (1.000) & (0.707) & (1.000) & (0.120) & (0.642)\\
F / L Height & 0.22 & -0.67 & -0.33 & -0.11 & -1.00 & 0.56 & -1.44 & -1.44 & -0.89 & 0.33 & -0.22 & -0.67 & -1.22 & -1.22 & -0.44 & 0.11 & -1.22 & 0.11 & 0.00 & -0.56 & 0.00\\
F / L Height (p) & (0.450) & (0.178) & (0.536) & (0.898) & (0.247) & (0.475) & (0.093) & (0.251) & (0.458) & (0.748) & (0.845) & (0.371) & (0.207) & (0.208) & (0.613) & (0.891) & (0.075) & (0.858) & (1.000) & (0.340) & (1.000)\\
\bottomrule
\end{tabular}


==> figuretable/birthday_project/ttest_receiver_serious_results.tex <==

\begin{tabular}[t]{lrrlrrlrrlrrlrrlrrlrrl}
\toprule
Receiver DB (Serious) & 25 & 26 & 27 & 28 & 29 & 30 & 31 & 32 & 33 & 34 & 35 & 36 & 37 & 38 & 39 & 40 & 41 & 42 & 43 & 44 & 45\\
\midrule
M / Total & 0.78 & 0.11 & 0.00 & 0.44 & 0.78 & -1.89 & 0.00 & 2.33 & 0.11 & 2.00 & 3.56 & -0.33 & -2.33 & 1.56 & 0.78 & -4.00 & -3.33 & 3.78 & 0.67 & 2.89 & -0.33\\
M / Total (p) & (0.015) & (0.862) & (1.000) & (0.719) & (0.611) & (0.341) & (1.000) & (0.173) & (0.952) & (0.450) & (0.053) & (0.838) & (0.155) & (0.339) & (0.700) & (0.049) & (0.018) & (0.052) & (0.643) & (0.244) & (0.856)\\
M / H Age & 0.67 & -0.22 & -0.44 & 1.11 & 0.67 & 0.78 & 1.22 & 0.11 & 0.33 & 1.11 & 1.22 & 1.11 & 1.11 & 0.44 & 0.00 & -0.22 & -0.22 & 0.00 & 0.22 & -0.11 & 0.11\\
M / H Age (p) & (0.020) & (0.619) & (0.504) & (0.210) & (0.238) & (0.360) & (0.148) & (0.855) & (0.710) & (0.078) & (0.023) & (0.098) & (0.153) & (0.415) & (1.000) & (0.447) & (0.598) & (1.000) & (0.447) & (0.716) & (0.736)\\
M / NA & 0.11 & 0.11 & -0.33 & 0.11 & -0.22 & -0.44 & 0.56 & 0.11 & 0.56 & -0.22 & 0.89 & -0.22 & 0.00 & 0.78 & -1.11 & -0.78 & -0.11 & 1.00 & 0.33 & 0.89 & 0.22\\
M / NA (p) & (0.347) & (0.624) & (0.260) & (0.837) & (0.600) & (0.464) & (0.505) & (0.869) & (0.484) & (0.802) & (0.300) & (0.728) & (1.000) & (0.148) & (0.083) & (0.168) & (0.716) & (0.012) & (0.431) & (0.009) & (0.347)\\
M / L Age & 0.00 & 0.22 & 0.78 & -0.78 & 0.33 & -2.22 & -1.78 & 2.11 & -0.78 & 1.11 & 1.44 & -1.22 & -3.44 & 0.33 & 1.89 & -3.00 & -3.00 & 2.78 & 0.11 & 2.11 & -0.67\\
M / L Age (p) & (1.000) & (0.462) & (0.139) & (0.238) & (0.757) & (0.178) & (0.112) & (0.213) & (0.635) & (0.642) & (0.404) & (0.424) & (0.042) & (0.867) & (0.252) & (0.124) & (0.020) & (0.144) & (0.944) & (0.349) & (0.697)\\
M / H Income & 0.00 & 0.00 & -0.33 & 0.33 & 0.44 & -0.22 & 0.22 & 0.11 & -0.33 & 0.00 & 0.33 & -0.22 & -0.44 & 0.67 & -0.11 & -1.00 & -0.33 & 0.78 & -0.33 & 1.89 & 0.44\\
M / H Income (p) &  &  & (0.236) & (0.380) & (0.195) & (0.678) & (0.659) & (0.844) & (0.520) & (1.000) & (0.599) & (0.789) & (0.625) & (0.418) & (0.928) & (0.291) & (0.643) & (0.310) & (0.662) & (0.050) & (0.615)\\
M / L Income & 0.78 & 0.11 & 0.33 & 0.11 & 0.33 & -1.78 & -0.11 & 2.22 & 0.33 & 2.00 & 3.22 & -0.11 & -2.00 & 0.78 & 0.89 & -2.89 & -3.22 & 3.00 & 1.00 & 0.89 & -0.67\\
M / L Income (p) & (0.015) & (0.862) & (0.715) & (0.929) & (0.825) & (0.347) & (0.943) & (0.194) & (0.853) & (0.420) & (0.067) & (0.945) & (0.258) & (0.560) & (0.499) & (0.154) & (0.013) & (0.044) & (0.475) & (0.639) & (0.621)\\
M / H Height & 0.67 & 0.22 & 0.44 & 0.67 & 0.00 & -2.22 & -0.44 & 1.78 & 0.78 & 1.22 & 2.44 & -1.00 & -2.00 & 3.00 & 0.67 & -3.00 & -4.22 & 3.22 & 1.00 & 3.22 & 0.22\\
M / H Height (p) & (0.017) & (0.659) & (0.649) & (0.447) & (1.000) & (0.118) & (0.755) & (0.320) & (0.593) & (0.550) & (0.151) & (0.485) & (0.204) & (0.082) & (0.736) & (0.088) & (0.001) & (0.042) & (0.497) & (0.144) & (0.886)\\
M / L Height & 0.11 & -0.11 & -0.44 & -0.22 & 0.78 & 0.33 & 0.44 & 0.56 & -0.67 & 0.78 & 1.11 & 0.67 & -0.33 & -1.44 & 0.11 & -1.00 & 0.89 & 0.56 & -0.33 & -0.33 & -0.56\\
M / L Height (p) & (0.347) & (0.711) & (0.362) & (0.785) & (0.359) & (0.640) & (0.649) & (0.554) & (0.542) & (0.471) & (0.285) & (0.345) & (0.636) & (0.087) & (0.892) & (0.351) & (0.361) & (0.571) & (0.657) & (0.709) & (0.384)\\
F / Total & 1.44 & 2.11 & 0.44 & 0.11 & 1.67 & -0.33 & -2.56 & 0.56 & -0.11 & 2.67 & -5.78 & -4.22 & 1.22 & -3.78 & -0.89 & -2.56 & -1.00 & -1.11 & 0.00 & -1.56 & -0.33\\
F / Total (p) & (0.134) & (0.070) & (0.773) & (0.957) & (0.526) & (0.869) & (0.150) & (0.832) & (0.971) & (0.200) & (0.007) & (0.016) & (0.447) & (0.024) & (0.644) & (0.215) & (0.476) & (0.411) & (1.000) & (0.221) & (0.634)\\
F / H Age & 1.44 & 1.89 & 0.00 & -0.78 & 2.11 & 1.11 & -2.33 & 1.56 & 1.33 & 2.89 & -3.78 & -3.44 & 2.33 & -2.22 & 0.44 & -1.56 & 0.22 & -1.11 & 0.44 & -0.78 & 0.00\\
F / H Age (p) & (0.119) & (0.078) & (1.000) & (0.690) & (0.347) & (0.488) & (0.223) & (0.489) & (0.510) & (0.167) & (0.073) & (0.057) & (0.109) & (0.183) & (0.803) & (0.358) & (0.819) & (0.311) & (0.616) & (0.435) & (1.000)\\
F / NA & 0.11 & 0.22 & 0.78 & 0.56 & 0.44 & 0.00 & 0.67 & 0.44 & -0.78 & 1.11 & -1.00 & -0.33 & 0.78 & -0.44 & -0.11 & -0.11 & -0.22 & -0.11 & -0.33 & 0.00 & 0.33\\
F / NA (p) & (0.556) & (0.411) & (0.202) & (0.245) & (0.523) & (1.000) & (0.361) & (0.642) & (0.191) & (0.078) & (0.116) & (0.560) & (0.195) & (0.479) & (0.867) & (0.878) & (0.712) & (0.775) & (0.379) & (1.000) & (0.336)\\
F / L Age & -0.11 & 0.00 & -0.33 & 0.33 & -0.89 & -1.44 & -0.89 & -1.44 & -0.67 & -1.33 & -1.00 & -0.44 & -1.89 & -1.11 & -1.22 & -0.89 & -1.00 & 0.11 & -0.11 & -0.78 & -0.67\\
F / L Age (p) & (0.347) & (1.000) & (0.468) & (0.461) & (0.322) & (0.097) & (0.442) & (0.104) & (0.569) & (0.190) & (0.092) & (0.675) & (0.033) & (0.171) & (0.040) & (0.339) & (0.116) & (0.874) & (0.867) & (0.182) & (0.067)\\
F / H Income & 0.56 & 0.78 & 1.33 & -1.78 & 1.78 & 0.89 & -1.78 & 0.00 & 0.11 & 1.56 & -3.22 & -4.33 & 1.11 & -2.22 & 0.11 & -1.11 & 0.89 & 0.22 & -0.56 & -0.22 & 0.00\\
F / H Income (p) & (0.333) & (0.347) & (0.227) & (0.178) & (0.159) & (0.550) & (0.165) & (1.000) & (0.953) & (0.267) & (0.085) & (0.010) & (0.415) & (0.023) & (0.928) & (0.403) & (0.446) & (0.777) & (0.539) & (0.816) & (1.000)\\
F / L Income & 0.89 & 1.33 & -0.78 & 1.78 & -0.11 & -1.22 & -0.78 & 0.56 & -0.22 & 1.00 & -2.56 & 0.11 & 0.22 & -1.56 & -1.00 & -1.44 & -1.89 & -1.33 & 0.56 & -1.33 & -0.33\\
F / L Income (p) & (0.162) & (0.158) & (0.489) & (0.307) & (0.954) & (0.514) & (0.531) & (0.757) & (0.890) & (0.559) & (0.061) & (0.921) & (0.789) & (0.323) & (0.397) & (0.326) & (0.047) & (0.205) & (0.618) & (0.158) & (0.570)\\
F / H Height & 1.00 & 2.11 & 0.22 & -0.11 & 1.89 & -0.11 & -1.22 & 1.44 & 1.67 & 1.67 & -5.11 & -3.44 & 0.89 & -2.22 & -0.56 & -3.11 & 0.44 & -0.67 & 0.56 & -1.44 & -0.44\\
F / H Height (p) & (0.188) & (0.034) & (0.839) & (0.946) & (0.405) & (0.953) & (0.463) & (0.502) & (0.461) & (0.291) & (0.007) & (0.078) & (0.593) & (0.150) & (0.730) & (0.032) & (0.740) & (0.535) & (0.534) & (0.206) & (0.346)\\
F / L Height & 0.44 & 0.00 & 0.22 & 0.22 & -0.22 & -0.22 & -1.33 & -0.89 & -1.78 & 1.00 & -0.67 & -0.78 & 0.33 & -1.56 & -0.33 & 0.56 & -1.44 & -0.44 & -0.56 & -0.11 & 0.11\\
F / L Height (p) & (0.284) & (1.000) & (0.814) & (0.863) & (0.851) & (0.845) & (0.320) & (0.515) & (0.269) & (0.449) & (0.612) & (0.435) & (0.778) & (0.165) & (0.717) & (0.548) & (0.033) & (0.576) & (0.378) & (0.819) & (0.860)\\
\bottomrule
\end{tabular}

